Sample-based Approximation of Nash in Large Many-Player Games via Gradient Descent

Nash equilibrium is a central concept in game theory. Several Nash solvers exist, yet none scale to normal-form games with many actions and many players, especially those with payoff tensors too big to be stored in memory. In this work, we propose an approach that iteratively improves an approximation to a Nash equilibrium through joint play. It accomplishes this by tracing a previously established homotopy that defines a continuum of equilibria for the game regularized with decaying levels of entropy. This continuum asymptotically approaches the limiting logit equilibrium, proven by McKelvey and Palfrey (1995) to be unique in almost all games, thereby partially circumventing the well-known equilibrium selection problem of many-player games. To encourage iterates to remain near this path, we efficiently minimize average deviation incentive via stochastic gradient descent, intelligently sampling entries in the payoff tensor as needed. Monte Carlo estimates of the stochastic gradient from joint play are biased due to the appearance of a nonlinear max operator in the objective, so we introduce additional innovations to the algorithm to alleviate gradient bias. The descent process can also be viewed as repeatedly constructing and reacting to a polymatrix approximation to the game. In these ways, our proposed approach, average deviation incentive descent with adaptive sampling (ADIDAS), is most similar to three classical approaches, namely homotopy-type, Lyapunov, and iterative polymatrix solvers. The lack of local convergence guarantees for biased gradient descent prevents guaranteed convergence to Nash, however, we demonstrate through extensive experiments the ability of this approach to approximate a unique Nash in normal-form games with as many as seven players and twenty one actions (several billion outcomes) that are orders of magnitude larger than those possible with prior algorithms.

==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,bbm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

%colored changes

\usepackage{cancel}
\def\colch#1{\textcolor{green}{{#1}}}

\usepackage{listings}
\usepackage{enumerate}

% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\usepackage{amsthm}

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\newtheorem{theorem}{Theorem}
\newreptheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}{Lemma}
\newreptheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\newcommand\myeq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}}

\newcommand{\tr}{^{\top}}

\newcommand{\assign}[2]{%
  \mathrel{#1}\mathrel{#2}%
}

==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/sections/01-intro.tex <==
\section{Introduction}
\label{intro}

% \ian{acknowledge history of nash with aaai/ijcai refs}
% \citep{lemke1964equilibrium,sandholm2005mixed,porter2008simple}

% \citep{govindan2003global,blum2006continuation}

% \citep{nudelman2004run}
Core concepts from game theory underpin many advances in multi-agent systems research. Among these, Nash equilibrium is particularly prevalent. Despite the difficulty of computing a Nash equilibrium~\citep{daskalakis2009complexity,chen2009settling}, a plethora of algorithms~\citep{lemke1964equilibrium,sandholm2005mixed,porter2008simple,govindan2003global,blum2006continuation} and suitable benchmarks~\citep{nudelman2004run} have been developed, however, none address large normal-form games with many actions and many players, especially those too big to be stored in memory.
% additional Nash complexity citation: chen2006settling
% zig-zag, not zig-zag-zig

% Game theory --> multiagent research / AI
% NE is central to 
% Nash is important
% \citep{daskalakis2009complexity,chen2006settling}

In this work, we develop an algorithm for approximating a Nash equilibrium of a normal-form game with so many actions and players that only a small subset of the possible outcomes in the game can be accessed at a time. We refer the reader to~\citet{mckelvey1996computation} for a review of approaches for normal-form games. Several algorithms exactly compute a Nash equilibrium for small normal-form games and others efficiently approximate Nash equilibria for special game classes, however, practical algorithms for approximating Nash in large normal-form games with many players, e.g. 7, and many actions, e.g., 21, is lacking. Computational efficiency is of paramount importance for large games because a general normal-form game with $n$ players and $m$ actions contains $nm^n$ payoffs; simply enumerating all payoffs can be intractable and renders classical approaches ineligible. A common approach is to return the profile found by efficient no-regret algorithms that sample payoffs as needed~\citep{blum_mansour_2007} although~\citet{flokas2020no} recently proved that many from this family do not converge to mixed Nash equilibria in \emph{all} games, 2-player games included. 

% \textbf{Our Contribution:} We introduce stochastic optimization into a classical \emph{homotopy} approach resulting in an algorithm that avoids the need to work with the full payoff tensor all at once and is, to our knowledge, the first capable of practically approximating Nash in large (trillions of outcomes) many-player, many-action normal form games. We demonstrate our algorithm on 2, 3, 4, 5, 6, 7 and 10 player games (5 and 10 in Appx.~\ref{app:xtra_games}; others in \S\ref{exp}). We also perform various ablation studies of our proposed algorithm (Appx.~\ref{app:ablations}), compare against several baselines including solvers from the popular \texttt{Gambit} library (more in Appx.~\ref{app:morealgs}), and examine a range of domains (more in Appx.~\ref{app:xtra_games}).
% % additional reference text: von2002computing
% % 7*21^7 * (4 bytes per float32) means 50gb tensor for diplomacy
% % 3.5 mb for efficient representation (symmetric)

% % Starcraft~\citep{vinyals2019alphastar,vinyals2019grandmaster} ($2$-player) and Diplomacy~\citep{anthony2020learning,gray2020human} ($7$-player)

% not only are many-player, many-action games are large, they are hard to solve.
% In this context, many-players refers to more than 2 players. While significant progress has been made for various 2-player games, computing and understanding systems with many interacting parts is difficult and so less progress has been made for normal-form games with more than 2 players\footnote{While any n-player game can, in theory, be efficiently solved for approximate equilibria by reducing it to a two-player game, in practice this approach is not feasible for solving large games due to the blowups involved in the reductions. Details in Appx.~\ref{app:beyondtwo}.}.


% \section{Background}

% In this work, many-players refers to more than 2 players.
While significant progress has been made for computing Nash in 2-player normal-form games which can be represented as a \emph{linear} complementarity problem, the many-player setting induces a \emph{nonlinear} complementarity problem, which is ``often hopelessly impractical to solve exactly''~(\cite{shoham2008multiagent}, p. 105).\footnote{While any n-player game can, in theory, be efficiently solved for approximate equilibria by reducing it to a two-player game, in practice this approach is not feasible for solving large games due to the blowups involved in the reductions. Details in Appx.~\ref{app:beyondtwo}.} The combination of high dimensionality ($m^n$ vs $m^2$ distinct outcomes) and nonlinearity (utilities are degree-$n$ polynomials in the strategies vs degree-$2$) makes many-player games much more complex.

% In this context, many-players refers to more than 2 players. It is well known across science and engineering that there exists a phase-transition when moving to the dynamical interaction of 3 or more entities\footnote{While any n-player game can, in theory, be efficiently solved for approximate equilibria by reducing it to a two-player game, in practice this approach is not feasible for solving large games due to the blowups involved in the reductions. Details in Appx.~\ref{app:beyondtwo}.}. The Lorenz system, a simple model of atmospheric convection, is easily recognized by its butterfly phase portrait and is the canonical example of chaos. Likewise, the three-body problem, the motion of three planets governed by Newtonian physics, is known to have no closed form solution. Computing and understanding systems with many interacting parts is difficult.

% \ian{add footnote: any 3+ player game can be reduced in polynomial time to a 2-player non-zero-sum game that weakly approximates the nash of the original game. practically, still not computable. details in Appx.~\ref{nuances}.}
% \ian{beyond 2-player zero-sum}
% Contrast this with the advances made in the 2 player regime. Von-Neumann's celebrated minimax theorem applies to two-player, zero-sum games; there exists no extension to more than 2 players. Generative adversarial networks~\citep{goodfellow2014generative}, gradient temporal difference learning~\citep{liu2018proximal}, and other minimax formulations of machine learning problems can be more difficult than their 1-player (optimization) model counterparts to train, but have all seen improving success.

% Most recently, EigenGame~\citep{gemp2020eigengame} was proposed as an n-player, general-sum, differentiable game whose Nash equals the solution to an eigenvalue problem. The authors imposed a hierarchy to prune the many complex interactions allowing easy computation of the Nash. In this work, we consider n-player, general-sum, normal form games with no assumptions on the interactions.
% This lack of structure makes the problem difficult.

This more general problem arises in cutting-edge multiagent research when learning~\citep{gray2020human} and evaluating~\citep{anthony2020learning} agents in Diplomacy, a complex 7-player board game. \citet{gray2020human} used no-regret learning to approximate a Nash equilibrium of subsampled games, however, this approach is brittle as we show later in Figure~\ref{fig:noregfail}. In \cite{anthony2020learning}, five Diplomacy bots were ranked according to their mass under an approximate Nash equilibrium. We extend that work to encourage convergence to a particular Nash and introduce sampling along with several technical contributions to scale evaluation to 21 Diplomacy bots, a >1000-fold increase in meta-game size.

Equilibrium computation has been an important component of AI in multi-agent systems~\citep{shoham2008multiagent}. It has been (and remains) a critical component of super-human AI in poker~\citep{Bowling15Poker,Moravcik17DeepStack,Brown17Libratus,brown2020combining}. 
%An approximate equilibrium solver is critical to training multi-agent systems as demonstrated by the use of %the AlphaStar League to train an agent to beat humans at Starcraft~\citep{vinyals2019alphastar,vinyals2019grandmaster}.
As mentioned above, Nash computation also arises when strategically summarizing a larger domain by learning a lower dimensionality empirical game~\citep{wellman2006methods}; such an approach was used in the AlphaStar League, leading to an agent that beat humans in StarCraft~\citep{vinyals2019alphastar,vinyals2019grandmaster}.
Ultimately, this required solving for the Nash of a 2-player, 888-action game, which can take several seconds using state-of-the-art solvers on modern hardware. 
%One might expect that to achieve superhuman performance at Diplomacy, we will need to solve a 7-player, 888-action game.
In contrast, solving an empirical game of Diplomacy, e.g., a 7-player 888-action game, would naively take longer than the current age of the universe.
This is well beyond the size of any game we inspect here, however, we approximate the Nash of games several orders of magnitude larger than previously possible, thus taking a step towards this ambitious goal.
% 7*(888^7) / (436,117,076,900,000,000) / (2*888^2) * 30

\textbf{Our Contribution:} We introduce stochastic optimization into a classical \emph{homotopy} approach resulting in an algorithm that avoids the need to work with the full payoff tensor all at once and is, to our knowledge, the first algorithm generally capable of practically approximating a unique Nash equilibrium in large (billions of outcomes) many-player, many-action normal-form games. We demonstrate our algorithm on 2, 3, 4, 6, 7 and 10 player games (10 in Appx.~\ref{app:xtra_games}; others in \S\ref{exp}). We also perform various ablation studies of our algorithm (Appx.~\ref{app:ablations}), compare against several baselines including solvers from the popular \texttt{Gambit} library (more in Appx.~\ref{app:morealgs}), and examine a range of domains (more in Appx.~\ref{app:xtra_games}).
% additional reference text: von2002computing
% 7*21^7 * (4 bytes per float32) means 50gb tensor for diplomacy
% 3.5 mb for efficient representation (symmetric)

% Starcraft~\citep{vinyals2019alphastar,vinyals2019grandmaster} ($2$-player) and Diplomacy~\citep{anthony2020learning,gray2020human} ($7$-player)

The paper is organized as follows. After formulating the Nash equilibrium problem for a general $n$-player normal-form game, we review previous work.
% One family of approaches in particular, namely homotopy methods, form the foundation of our algorithm. We extend the ideas there by incorporating \emph{stochastic} optimization, thereby avoiding computing all possible payoffs in the game by sampling payoffs as needed.
We discuss how we combine the insights of classical algorithms with ideas from stochastic optimization to develop our final algorithm, \emph{average deviation incentive descent with adaptive sampling}, or ADIDAS.
Finally, we compare our proposed algorithm against previous approaches on large games of interest from the literature: games such as Colonel Blotto~\citep{arad2012multi}, classical Nash benchmarks from the GAMUT library~\citep{nudelman2004run}, and games relevant to recent success on the $7$-player game Diplomacy~\citep{anthony2020learning,gray2020human}.
% diplomacy citation: calhamer1959diplomacy
% blotto 2nd citation: borel1953theory
% \ian{these games are deceptively complex challenge domains - recent soda papers}
% \ian{we put together many known ideas}

==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/sections/02-problem.tex <==
% \ian{rename next two sections to preliminaries}

% \section{$n$-Player Normal-Form Games}
\section{Preliminaries}
% \begin{align}
%     \max_{x_i \in \Delta^{m_i-1}} \{u_i(x_i,x_{-i}) = T^{(i)}_{a_1 \ldots a_n} x_{1a_1} \ldots x_{na_n} \} \label{i_obj}
% \end{align}
% where $T^{(i)}$ is the $n$-dimensional payoff tensor for player $i$ with shape $(m_1 \times \ldots \times m_n)$, $\Delta^{m_i-1}$ is the $(m_i-1)$-dimensional simplex embedded in $\mathbb{R}^m_i$, $x_{ia_i}$ is the probability of player $i$ taking action $a_i$, and $x_{-i}$ denotes all strategies belonging to players other than player $i$. A joint strategy $\boldsymbol{x} = [x_1, \ldots, x_n]$ is a Nash equilibrium if and only if each $x_i$ solves~\eqref{i_obj}, i.e., $x_i$ is a maximizer of $u_i(x_i, x_{-i})$.
In a finite $n$-player game in normal form, each player $i \in \{1,\ldots,n\}$ is given a strategy set $\mathcal{A}_i = \{a_{i1}, \ldots, a_{im_i}\}$ consisting of $m_i$ pure strategies. The pure strategies can be naturally indexed by non-negative integers, so we redefine $\mathcal{A}_i = \{0, \ldots, m_i - 1\}$ as an abuse of notation for convenience. Each player $i$ is also given a payoff or utility function, $u_i: \mathcal{A} \rightarrow \mathbb{R}$ where $\mathcal{A} = \prod_i \mathcal{A}_i$. In games where the cardinality of each player's strategy set is the same, we drop the subscript on $m_i$. Player $i$ may play a mixed strategy by sampling from a distribution over their pure strategies. Let player $i$'s mixed strategy be represented by a vector $x_i \in \Delta^{m_i-1}$ where $\Delta^{m_i-1}$ is the $(m_i-1)$-dimensional probability simplex embedded in $\mathbb{R}^{m_i}$. Each function $u_i$ is then extended to this domain so that $u_i(\boldsymbol{x}) = \sum_{\boldsymbol{a} \in \mathcal{A}} u_i(\boldsymbol{a}) \prod_{j} x_{ja_j}$ where $\boldsymbol{x} = (x_1, \ldots, x_n)$ and $a_j \in \mathcal{A}_j$ denotes player $j$'s component of the joint action $\boldsymbol{a} \in \mathcal{A}$. For convenience, let $x_{-i}$ denote all components of $\boldsymbol{x}$ belonging to players other than player $i$.

We say $\boldsymbol{x} \in \prod_i \Delta^{m_i-1}$ is a Nash equilibrium iff, for all $i \in \{1, \ldots, n\}$, $u_i(z_i, x_{-i}) \le u_i(\boldsymbol{x})$ for all $z_i \in \Delta^{m_i-1}$, i.e., no player has any incentive to unilaterally deviate from $\boldsymbol{x}$. Nash is most commonly relaxed with $\epsilon$-Nash, an additive approximation: $u_i(z_i, x_{-i}) \le u_i(\boldsymbol{x}) + \epsilon$ for all $z_i \in \Delta^{m_i-1}$. Later we explore the idea of regularizing utilities with a function $S^{\tau}_i$ (e.g., entropy) as follows:% $u^{\tau}_i(\boldsymbol{x}) = u_i(\boldsymbol{x}) + S^{\tau}_i(x_i, x_{-i})$.
\begin{align}
    u^{\tau}_i(\boldsymbol{x}) &= u_i(\boldsymbol{x}) + S^{\tau}_i(x_i, x_{-i}).
\end{align}

As an abuse of notation, let the atomic action $a_{i}$ also denote the $m_i$-dimensional ``one-hot" vector with all zeros aside from a $1$ at index $a_{i}$; its use should be clear from the context. And for convenience, denote by $H^i_{il} = \mathbb{E}_{x_{-il}}[u_i(a_i, a_l, x_{-il})]$ the Jacobian\footnote{See Appx.~\ref{appx:nfg_grad} for an example derivation of the gradient if this form is unfamiliar.} of player $i$'s utility with respect to $x_i$ and $x_l$; $x_{-il}$ denotes all strategies belonging to players other than $i$ and $l$ and $u_i(a_i, a_l, x_{-il})$ separates out $l$'s strategy $x_l$ from the rest of the players $x_{-i}$. We also introduce $\nabla^i_{x_i}$ as player $i$'s utility gradient. Note player $i$'s utility can now be written succinctly as $u_i(x_i, x_{-i}) = x_i^\top \nabla^i_{x_i} = x_i^\top H^i_{il} x_l$ for any $l$.

In a polymatrix game, interactions between players are limited to local, pairwise games, each of which is represented by matrices $H^i_{ij}$ and $H^j_{ij}$. This reduces the exponential $nm^n$ payoffs required to represent a general normal form game to a quadratic $n(n-1)m^2$, an efficiency we leverage later.

% \ian{In a polymatrix game, only pairwise interactions between players are modeled $H^i_{ij}$ and $H^j_{ij}$. $\epsilon$-Nash is an additive approximation. Polymatrix is quadratic rather than exponential, which our algorithm leverages.}

% (also called policy gradient)


==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/sections/03-related_work.tex <==
\subsection{Related work}
% \label{related_work}

Several approaches exist for computing Nash equilibria of $n$-player normal form games\footnote{Note that Double-Oracle~\citep{mcmahan2003planning} and PSRO~\citep{lanctot2017unified} can be extended to n-player games, but require an n-player normal form meta-solver (Nash-solver) and so cannot be considered solvers in their own right. This work provides an approximate meta-solver.}. Simplicial Subdivision (SD)~\citep{van1987simplicial} searches for an equilibrium over discretized simplices; accuracy depends on the grid size which scales exponentially with the number of player actions. \citet{govindan2003global} propose a homotopy method (GW) that begins with the unique Nash distribution of a game whose payoff tensor has been perturbed by an arbitrary constant tensor. GW then scales back this perturbation while updating the Nash to that of the transformed game. GW is considered an extension of the classic Lemke-Howson algorithm (\citeyear{lemke1964equilibrium}) to $3$+ player games (see \S4.3, p. 107 of ~\citep{shoham2008multiagent}).
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/AlgComparison_LastNameYear.pdf}
    \caption{Algorithm Comparison and Overview.}
    \label{fig:algcomp}
\end{figure}
Another homotopy approach perturbs the payoffs with entropy bonuses, and evolves the Nash distribution along a continuum of quantal response equilibria (QREs) using a predictor-corrector method to integrate a differential equation~\citep{turocy2005dynamic} \textemdash we also aim to follow this same continuum. In a slightly different approach,~\citet{perolat2020poincar} propose an adaptive regularization scheme that repeatedly solves for the equilibrium of a transformed game. Simple search methods~\citep{porter2008simple} that approach Nash computation as a constraint satisfaction problem appear to scale better than GW and SD as measured on GAMUT benchmarks~\citep{nudelman2004run}. Lyapunov approaches minimize non-convex energy functions with the property that zero energy implies Nash~\citep{shoham2008multiagent}, however these approaches may suffer from convergence to local minima with positive energy. In some settings, such as polymatrix games with payoffs in $[0, 1]$, gradient descent on appropriate energy functions\footnote{\Eqref{popexp} but with $\max$ instead of $\sum$ over player regrets. Note that for symmetric games with symmetric equilibria, these are equivalent up to a multiplicative factor $n$.} guarantees a $(\frac{1}{2} + \delta)$-Nash in time polynomial in $\frac{1}{\delta}$~\citep{deligkas2017computing} and performs well in practice~\citep{deligkas2016empirical}.

\paragraph{Teaser} Our proposed algorithm consists of two key conceptual schemes. One lies at the crux of homotopy methods (see Figures~\ref{fig:algcomp} and~\ref{fig:homotopy}). We initialize the Nash approximation, $\boldsymbol{x}$, to the joint uniform distribution, the unique Nash of a game with infinite-temperature entropy regularization. The temperature is then annealed over time. To recover the Nash at each temperature, we minimize an appropriately adapted energy function via (biased) stochastic gradient descent. This minimization approach can be seen as simultaneously learning a suitable polymatrix decomposition of the game similarly to~\citet{govindan2004computing} but from batches of stochastic play, i.e., we compute Monte Carlo estimates of the payoffs in the bimatrix game between every pair of players by observing the outcomes of the players' joint actions (sampled from $\boldsymbol{x}$ after each update) rather than computing payoffs as exact expectations.
% VIs
\nocite{facchinei2007finite}
% MIP approach
\nocite{sandholm2005mixed}
% Graphical Game Homotopy type
\nocite{blum2006continuation}
% GW'04 looks at a 4player 10action game which is 1242 times smaller than Diplomacy 7-21

% For completeness, we also consider solvers that compute correlated equilibria. In order to compare to Nash, we factorize the correlated equilibrium as an approximation. A correlated equilibrium can be formulated as a linear program, for which fast solvers exist, so it is worth considering. 

% \begin{itemize}
%     \item classical deterministic solvers: lp approaches, csp approaches, homotopy method, lyapunov approaches, discretization approaches
%     \item psro + classical solvers
%     \begin{itemize}
%         \item Double-Oracle algorithm~\citep{mcmahan2003planning}
%         \item 2-player zero-sum perfect-information~\citep{lanctot2017unified}
%         \item 2-player zero-sum \emph{imperfect}-information~\citep{mcaleer2020pipeline}
%         \item $N$-player general-sum perfect-information [this work] (openAI-5, 5v5)
%     \end{itemize}
%     \item correlated eq solvers + brute factorization
%     \item ours is homotopy + laypunov (+ stochastic)
% \end{itemize}

% \begin{enumerate}
%     \item Simplicial Subdivision~\citep{van1987simplicial} (discretizes the simplex) and Govindan-Wilson~\citep{govindan2003global} (nash): GW is a global newton method implemented in Gambit (approx 53k hrs for blotto problem - \url{https://github.com/gambitproject/gambit/issues/261#issuecomment-660894391}). GW is also considered an extension of Lemke-Howson~\citep{lemke1964equilibrium} to 2+ player (p. 107 of~\citep{shoham2008multiagent}).
%     \item Simple search method for Nash~\citep{porter2008simple}. Buggy code in Haskel here: \url{https://github.com/spgarbet/sample-nash}.
%     \item no-regret learners + averaging (coarse correlated)
%     \item LP-solvers (correlated)
%     \item MCCFR in extensive form games (Nash) and Pipeline PSRO in extensive form (Nash)
%     \item Gambit solvers - none appear fit to run on very large games. gambit-logit~\citep{turocy2005dynamic} is best prepared, but even in the paper, max player is 5 (5,2) and max actions is 20 (2,20). gambit-logit still takes forever (gambit-logit lambda=1.02 qre solution after 101minutes with nash-conv = 0.0656848861190602). prob worth rerunning: \begin{verbatim}time gambit-logit -m 1 -e < ~/gambit/nfgs/blotto_10_3_4.nfg\end{verbatim}. stochastic version of gambit-logit may be possible but that seems to be unexplored territory.
% \end{enumerate}

==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/sections/04-method.tex <==
\section{Deviation Incentive \& Warm-Up}

% \ian{move pop exp to intro with connection to $\epsilon$-Nash} \textcolor{red}{you sure it can't just stay here?}

We propose minimizing the energy function in~\eqref{popexp} below, \emph{average deviation incentive} (ADI), to approximate a Nash equilibrium of a large, entropy-regularized normal form game. This loss measures, on average, how much a single agent can exploit the rest of the population by deviating from a joint strategy $\boldsymbol{x}$. For sake of exposition, we drop the normalizing constant from the denominator (number of players, $n$), and consider the sum instead of the average. This quantity functions as a \emph{loss} that can be minimized over $\mathcal{X} = \prod_i \Delta^{m_i-1}$ to find a Nash distribution. Note that when ADI is zero, $\boldsymbol{x}$ is a Nash. Also, if $\sum_k$ is replaced by $\max_k$, this loss measures the $\epsilon$ of an $\epsilon$-Nash, and therefore,~\eqref{popexp} is an upper bound on this $\epsilon$.  Lastly, note that, in general, this loss function is non-convex and so convergence to local, suboptimal minima is theoretically possible if naively minimizing via first order methods like gradient descent \textemdash we explain in \S\ref{annealing} how we circumvent this pitfall via temperature annealing. Let $\br_k = \br(x_{-k}) = \argmax_{z_k \in \Delta^{m_k-1}} u^{\tau}_k(z_k, x_{-k})$ be player $k$'s best response to all other players' current strategies where $u^\tau_k$ is player $k$'s utility regularized by entropy with temperature $\tau$ and formally define
\begin{align}
    \mathcal{L}^{\tau}_{adi}(\boldsymbol{x}) &= \sum_k \overbrace{u^{\tau}_k(\br_k, x_{-k}) - u^{\tau}_k(x_k,x_{-k})}^{\text{incentive to deviate to $\br_k$ vs $\boldsymbol{x}_k$}}. \label{popexp}
\end{align}

% where
% \begin{align}
%     \br_k &= \br(x_{-k}) = \argmax_{z_k \in \Delta^{m_k-1}} u^{\tau}_k(z_k, x_{-k})
% \end{align}
If $\tau=0$, we drop the superscript and use $\mathcal{L}_{adi}$. The Nash equilibrium of the game regularized with Shannon entropy is called a \emph{quantal response equilibrium}, QRE($\tau$) (see p. 152-154, 343 of~\cite{fudenberg1998theory}).
% 2-player reference for QRE as entropy bonus is \cite{ling2018game}
% Also, we define $\argmax$ so it distributes weight uniformly over the ``best-responses", e.g., $\argmax ([1, 1, 0]) = [\frac{1}{2}, \frac{1}{2}, 0]$.\footnote{This definition of $\argmax$ is not critical; it simply better matches our entropy regularized versions in the zero temperature limit.}

Average deviation incentive has been interpreted as a pseudo-distance from Nash in prior work, where it is referred to as \texttt{NashConv} \citep{lanctot2017unified}. We prefer average deviation incentive because it more precisely describes the function and allows room for exploring alternative losses in future work. The objective can be decomposed into terms that depend on $x_k$ (second term) and $x_{-k}$ (both terms). Minimizing the second term w.r.t. $x_k$ seeks strategies with high utility, while minimizing both terms w.r.t. $x_{-k}$ seeks strategies that cannot be exploited by player $k$. In reducing $\mathcal{L}_{adi}$, each player $k$ seeks a strategy that not only increases their payoff but also removes others' temptation to exploit them.

A related algorithm is Exploitability Descent (ED)~\citep{Lockhart19ED}.
% Rather than optimizing~\eqref{popexp} directly, player $k$ $\mathcal{L}^\tau_{adi}$ each player's strategy is adjusted using a gradient ascent against the best-responding opponent(s).
Rather than minimizing $\mathcal{L}_{adi}$, each player independently maximizes their utility assuming the other players play their best responses. In the two-player normal-form setting, ED is equivalent to extragradient~\citep{korpelevich1976extragradient}~(see Appx.~\ref{app:ed_connection}). However, ED is only guaranteed to converge to Nash in two-player, zero-sum games. We include a comparison against ED as well as Fictitious-play, another popular multiagent algorithm, in Appx.~\ref{app:xtra_comparisons}. We also relate $\mathcal{L}_{adi}$ to Consensus optimization~\citep{mescheder2017numerics} in Appx.~\ref{app:consensus_connection}.

% Previous work performs gradient descent on this loss to solve for Nash~\citep{anthony2020learning}. In that work, expectations of random variables are computed exactly requiring all entries in the payoff tensor. In this work, we develop a stochastic version of this solver that scales to larger games.

% \ian{move connection to dip solver to experiments / conclusion}

\subsection{Warm-Up}
\label{annealing}
% As mentioned in the related work, our approach is similar to Lyapunov approaches which typically suffer from convergence to local minima. If we were to naively minimize $\mathcal{L}_{adi}$, we might also suffer from this issue. However, we incorporate techniques from homotopy approaches to avoid this issue.
\citet{mckelvey1995quantal} proved the existence of a continuum of QREs starting at the uniform distribution (infinite temperature) and ending at what they called the \emph{limiting logit equilibrium} (LLE). Furthermore, they showed this path is unique for \emph{almost all games}, partially circumventing the equilibrium selection problem. We encourage the reader to look ahead at Figure~\ref{fig:homotopy} for a visual of the homotopy that may prove helpful for the ensuing discussions.

In this work, we assume we are given one of these common games with a unique path (no branching points) so that the LLE is well defined (\textbf{Assumption~\ref{nobranches}}). Furthermore, we assume there exist no ``turning points'' in the temperature $\tau$ along the continuum (\textbf{Assumption~\ref{noturning}}). \citet{turocy2005dynamic} explains that even in generic games, temperature might have to be temporarily increased in order to remain on the path (principal branch) to the LLE. However, \citeauthor{turocy2005dynamic} also proves there exists a $\tau^*$ such that no turning points exist with $\tau > \tau^*$ suggesting that as long as we remain near the principal branch after $\tau^*$, we can expect to proceed to the LLE.

We follow the principal path by alternating between annealing the temperature and re-solving for the Nash at that temperature by minimizing $\mathcal{L}^{\tau}_{adi}$. We present a basic version of our approach that converges to the limiting logit equilibrium assuming access to exact gradients in Algorithm~\ref{alg_warmup} (proof in Appx.~\ref{app:conv}). We substitute $\lambda=\frac{1}{\tau}$ and initialize $\lambda=0$ in order to begin at infinite temperature. The proof of this simple warm-up algorithm relies on the detailed examination of the continuum of QREs proposed in~\cite{mckelvey1995quantal} and further analyzed in~\cite{turocy2005dynamic}. Theorem~\ref{conv_basic} presented below is essentially a succinct repetition of one of their known results (Assumptions~\ref{sensitivity} and~\ref{boa} below are expanded on in Appx.~\ref{app:conv}). In subsequent sections, we relax the exact gradient assumption and assume gradients are estimated from stochasic play (i.e., each agent samples an action from their side of the current approximation to the Nash).

\begin{algorithm}[H]
\begin{algorithmic}[1]
    \STATE Given: Total anneal steps $T_{\lambda}$, total optimizer iterations $T^*$, and anneal step size $\Delta \lambda$.
    \STATE $\lambda = 0$
    \STATE $\boldsymbol{x} \leftarrow \{ \frac{1}{m_i} \boldsymbol{1} \,\, \forall \,\, i\}$
    \FOR{$t_{\lambda} = 1: T_{\lambda}$}
        \STATE $\lambda \leftarrow \lambda + \Delta \lambda$ \label{line:anneal}
        \STATE $\boldsymbol{x} \leftarrow \texttt{OPT}(\texttt{loss} = \mathcal{L}^{\tau=\lambda^{-1}}_{adi}, \boldsymbol{x}_{init} = \boldsymbol{x}, iters = T^*)$ \label{line:descend}
    \ENDFOR
    \STATE return $\boldsymbol{x}$
\end{algorithmic}
\caption{Warm-up: Anneal \& Descend}
\label{alg_warmup}
\end{algorithm}

\begin{theorem}
\label{conv_basic}
Make assumptions~\ref{nobranches} and~\ref{noturning}. Also, assume the QREs along the homotopy path have bounded sensitivity to $\lambda$ given by a parameter $\sigma$ (Assumption~\ref{sensitivity}), and basins of attraction with radii lower bounded by $r$ (Assumption~\ref{boa}). Let the step size $\Delta \lambda \le \sigma (r - \epsilon)$ with tolerance $\epsilon$. And let $T^*$ be the supremum over all $T$ such that Assumption~\ref{boa} is satisfied for any inverse temperature $\lambda \ge \Delta \lambda$. Then, assuming gradient descent for \texttt{OPT}, \Algref{alg_warmup} converges to the limiting logit equilibrium $\boldsymbol{x}^*_{\lambda=\infty} = \boldsymbol{x}^*_{\tau=0}$ in the limit as $T_{\lambda} \rightarrow \infty$.
\end{theorem}

\subsection{Evaluating $\mathcal{L}^{\tau}_{adi}$ with Joint Play}
\label{bias_intuition}

% \ian{go more slowly here on this example} \textcolor{red}{is this better?}

In the warm up, we assumed we could compute exact gradients which required access to the entire payoff tensor. However, we want to solve very large games where enumerating the payoff tensor is prohibitively expensive. Therefore, we are particularly interested in minimizing $\mathcal{L}^{\tau}_{adi}$ when only given access to samples of joint play, $\boldsymbol{a} \sim \prod_i x_i$. The best response operator, $\br$, is nonlinear and hence can introduce bias if applied to random samples. For example, consider the game given in Table~\ref{tab:biased_game} and assume $x_2 = [0.5, 0.5]^\top$.

% \begin{figure}[ht!]
% \begin{minipage}{0.5\textwidth}
% \begin{table}[ht!]
%     \centering
%     \begin{tabular}{c|c|c}
%         $u_1$ & $a_{21}$ & $a_{22}$ \\ \hline
%         $a_{11}$ & 0 & 0 \\
%         $a_{12}$ & 1 & -2 \\
%         $a_{13}$ & -2 & 1
%     \end{tabular}
%     \hspace{1.0cm}
%     \begin{tabular}{c|c|c}
%         $u_2$ & $a_{21}$ & $a_{22}$ \\ \hline
%         $a_{11}$ & 0 & 0 \\
%         $a_{12}$ & 0 & 0 \\
%         $a_{13}$ & 0 & 0
%     \end{tabular}
%     \begin{align}
%         br_1 &= blah
%         \\ br_2 &= blah 2
%     \end{align}
%     \caption{A 2-player game with biased stochastic $\br$'s.}
%     \label{tab:biased_game}
% \end{table}
% \begin{figure}
% \begin{floatrow}
% \capbtabbox{%
%   \begin{tabular}{c|c|c}
%         $u_1$ & $a_{21}$ & $a_{22}$ \\ \hline
%         $a_{11}$ & 0 & 0 \\
%         $a_{12}$ & 1 & -2 \\
%         $a_{13}$ & -2 & 1
%     \end{tabular}
%     \hspace{1.0cm}
%     \begin{tabular}{c|c|c}
%         $u_2$ & $a_{21}$ & $a_{22}$ \\ \hline
%         $a_{11}$ & 0 & 0 \\
%         $a_{12}$ & 0 & 0 \\
%         $a_{13}$ & 0 & 0
%     \end{tabular}
% }{%
%   \caption{A 2-player game with biased stochastic $\br$'s.}%
% }
% \begin{minipage}{0.2\textwidth}
% \begin{align}
%         \mathbb{E}[\br{}^{\tau\rightarrow 0}] &= [0.00, 0.50, 0.50]
%         \\ \mathbb{E}[\br{}^{\tau=1}] &\approx [0.26, 0.37, 0.37]
%         \\ \mathbb{E}[\br{}^{\tau=10}] &= [0.42, 0.29, 0.29]
% \end{align}
% \end{minipage}
% \end{floatrow}
% \end{figure}
\begin{table}[!ht]
% \begin{minipage}{0.5\textwidth}
    \centering
    \begin{tabular}{c|c|c}
        $u_1$ & $a_{21}$ & $a_{22}$ \\ \hline
        $a_{11}$ & 0 & 0 \\
        $a_{12}$ & 1 & -2 \\
        $a_{13}$ & -2 & 1
    \end{tabular}
    \hspace{1.0cm}
    \begin{tabular}{c|c|c}
        $u_2$ & $a_{21}$ & $a_{22}$ \\ \hline
        $a_{11}$ & 0 & 0 \\
        $a_{12}$ & 0 & 0 \\
        $a_{13}$ & 0 & 0
    \end{tabular}
    \caption{A 2-player game with biased stochastic $\br$'s.}
    \label{tab:biased_game}
% \end{minipage}
% \begin{minipage}{0.5\textwidth}
%     \centering
%     \begin{align}
%             \mathbb{E}[\br{}^{\tau\rightarrow 0}] &= [0.00, 0.50, 0.50] \label{zero_temp}
%             \\ \mathbb{E}[\br{}^{\tau=1}] &\approx [0.26, 0.37, 0.37]
%             \\ \mathbb{E}[\br{}^{\tau=10}] &\approx [0.42, 0.29, 0.29] \label{goldilocks}
%             % \\ \mathbb{E}[\br{}^{\tau\rightarrow\infty}] &= [0.33, 0.33, 0.33]
%     \end{align}
% \end{minipage}
\end{table}
% \end{minipage}
% \begin{minipage}{0.5\textwidth}
%     \begin{align}
%         br_1 &= blah
%     \end{align}
% \end{minipage}
% \end{figure}
%
% \begin{align}
%     % u_1(x_1, x_2) &= \begin{bmatrix} x_{1a_0} & x_{1a_1} & x_{1a_2} \end{bmatrix} \begin{bmatrix}
%     % 0 & 0 \\
%     % 1 & -2 \\
%     % -2 & 1
%     % \end{bmatrix} \begin{bmatrix} x_{2a_0} \\ x_{2a_1} \end{bmatrix}.
%     u_1(x_1, x_2) &= x_1^\top \begin{bmatrix}
%     0 & 0 \\
%     1 & -2 \\
%     -2 & 1
%     \end{bmatrix} x_2 = x_1^\top  H^1_{12} x_2.
% \end{align}
%
Consider computing (row) player $1$'s best response to a single action sampled from (column) player $2$'s strategy $x_2$. Either $a_{21}$ or $a_{22}$ will be sampled with equal probability, which results in a best response of either $a_{12}$ or $a_{13}$ respectively. However, the true expected utilities for each of player $1$'s actions given player $2$'s strategy are $[0, -0.5, -0.5]$ for which the best response is the first index, $a_{11}$. The best response operator completely filters out information on the utility of the true best response $a_{11}$. Intuitively, a \emph{soft} best response operator, demonstrated in equations (\ref{zero_temp})-(\ref{goldilocks}), that allows some utility information for each of the actions to pass through could alleviate the problem:
\begin{align}
    \mathbb{E}[\br{}^{\tau\rightarrow 0}] &= [0.00, 0.50, 0.50] \label{zero_temp}
    \\ \mathbb{E}[\br{}^{\tau=1}] &\approx [0.26, 0.37, 0.37]
    \\ \mathbb{E}[\br{}^{\tau=10}] &\approx [\mathbf{0.42}, 0.29, 0.29]. \label{goldilocks}
    % \\ \mathbb{E}[\br{}^{\tau\rightarrow\infty}] &= [0.33, 0.33, 0.33]
\end{align}
By adding an entropy regularizer to the utilities, $\tau \mathcal{H}(x_i)$, we induce a soft-$\br$. Therefore, the homotopy approach has the added benefit of partially alleviating gradient bias for moderate temperatures. Further empirical analysis of bias can be found in Appx.~\ref{appx:bias}.
% Therefore, careful attention must be made to account for the bias introduced in the stochastic setting.

% \ian{which lingo to use? actions vs pure strategies, joint strategies vs profiles, utilities vs payoffs...}

% \paragraph{Entropy alleviates bias} In the example above, the best response operator completely filters out information on the utility of the true best response $a_{11}$. Intuitively, a \emph{soft} best response operator that allows some utility information for each of the actions to pass through could alleviate the problem. We can induce a soft-$\br$ by adding an entropy regularizer to the utilities, $e.g., \tau \mathcal{H}(x_i)$. Note, however, that too much entropy can also destroy information. In the limit as $\tau \rightarrow \infty$, the best response approaches a constant vector completely filtering out information regarding \emph{all} actions. Later, we study the gradient bias problem empirically and demonstrate that entropy regularization can combat the issue.

% \textcolor{red}{add discusion around: motivation for entropy here is to maximize information gained after BR. in QRE, it models bounded rationality. annealing entropy models learning the game payoffs, refinement of strategies, etc.}

\section{ADIDAS}

In the previous section, we laid out the conceptual approach we take and identified bias as a potential issue to scaling up computation with Monte Carlo approximation. Here, we inspect the details of our approach, introduce further modifications to reduce the issue of bias, and present our resulting algorithm ADIDAS. Finally, we discuss the advantages of our approach for scaling to large games.

\subsection{Deviation Incentive Gradient}
\label{ped_grads}

% \ian{why two entropies? which is better?} \textcolor{red}{inconclusive. should i move ATE to the appendix then?}

% We now derive the gradient of average deviation incentive regularized with a Shannon entropy term. We also explore using an adaptive Tsallis entropy (\texttt{ATE}) in the appendix.
% either a tailored Tsallis or Shannon entropy term.

% \subsection{Shannon Entropy}
Regularizing the utilities with weighted Shannon entropy, $u^{\tau}_k(\boldsymbol{x}) = u_k(\boldsymbol{x}) + S^\tau_k(x_k, x_{-k})$, where $S^\tau_k(x_k, x_{-k}) = -\tau \sum_{a_k} x_{ka_k} \ln(x_{ka_k})$, leads to the following average deviation incentive gradient derived in Appx.~\ref{gen_pop_exp_grad} where $\br_j = \texttt{softmax}(\nabla^j_{x_j}/\tau)$ and $\texttt{diag}(v)$ creates a diagonal matrix with $v$ on the diagonal:
\begin{align}
    &\nabla_{x_i} \mathcal{L}^{\tau}_{adi}(\boldsymbol{x}) = -\overbrace{(\nabla^i_{x_i} - \tau (\ln(x_i) + 1))}^{\text{policy gradient}} \nonumber
    \\ &+ \sum_{j \ne i} \Big[ J_{x_i}(\br_j)^\top (\nabla^j_{x_j} - \tau (\ln(\br_j) + 1)) + H^j_{ij} (\br_j - x_j) \Big] \label{qre_grad}
    \\ &\text{with } J_{x_i}(\br_j) = \frac{1}{\tau} (\texttt{diag}(\br_j) - \br_j \br_j^\top) H^j_{ji}. \label{qre_jac}
\end{align}
% and
% \begin{align}
%     J_{x_i}(\br_j) &= \frac{1}{\tau} (\texttt{diag}(\br_j) - \br_j \br_j^\top) H^j_{ji}. \label{qre_jac}
% \end{align}
%
% \subsection{No Entropy}
In the limit, $\nabla_{x_i} \mathcal{L}^{\tau}_{adi}(\boldsymbol{x}) \stackrel{\tau\rightarrow 0^+}{=} -\nabla^i_{x_i} + \sum_{j \ne i} H^j_{ij} (\br_j - x_j)$. The first term is recognized as player $i$'s payoff or \emph{policy} gradient. The second term is a correction that accounts for the other players' incentives to exploit player $i$ through a strategy deviation.
% \begin{align}
%     &\nabla_{x_i} \mathcal{L}_{adi}(\boldsymbol{x}) \stackrel{\tau\rightarrow 0^+}{=} -\nabla^i_{x_i} + \sum_{j \ne i} H^j_{ij} (\br_j - x_j).
%     % = \sum_{j \ne i} H^j_{ij} (\br(x_{-j}) - x_j) - \frac{1}{n-1} H^i_{ij} x_j.
% \end{align}
% \footnote{Assuming we remove the $\boldsymbol{1} ||\nabla^i_{x_i}||_{\infty}$ component from the Tsallis entropy gradient.}
%
Each $H^j_{ij}$ approximates player $j$'s payoffs in the bimatrix game between players $i$ and $j$. Recall from the preliminaries that in a polymatrix game, these matrices capture the game exactly. We also explore an adaptive Tsallis entropy in Appx.~\ref{gen_pop_exp_grad}.

\subsection{Amortized Estimates with Historical Play}
\label{amortized_estimates}

% \ian{move simplified alg up and add more complex one to appendix}

Section~\ref{bias_intuition} discusses the bias that can be introduced when best responding to sampled joint play and how the annealing process of the homotopy method helps alleviate it by softening the $\br$ operator with entropy regularization. To reduce the bias further, we could evaluate more samples from $\boldsymbol{x}$, however, this increases the required computation. Alternatively, assuming strategies have changed minimally over the last few updates (i.e., $\boldsymbol{x}^{(t-2)} \approx \boldsymbol{x}^{(t-1)} \approx \boldsymbol{x}^{(t)}$), we can instead reuse historical play to improve estimates. We accomplish this by introducing an auxiliary variable $y_i$ that computes an exponentially averaged estimate of each player $i$'s payoff gradient $\nabla^i_{x_i}$ throughout the descent similarly to~\citet{sutton2008convergent}.
% \footnote{Similar ideas are used in Gradient TD (RL)~\citep{sutton2008convergent}.}.
% \nocite{sutton2008convergent}
%
We also use $y_i$ to compute an estimate of ADI, $\hat{\mathcal{L}}^{\tau}_{adi}$, as follows:
\begin{align}
    \hat{\mathcal{L}}^{\tau}_{adi}(\boldsymbol{x}, \boldsymbol{y}) &= \sum_k y_k^\top (\hat{\br}_k - x_k) +  S^\tau_k(\hat{\br}_k, x_{-k}) - S^\tau_k(x_k, x_{-k}) \label{amortized_exp_reg}
\end{align}
where $\hat{\br}_k = \argmax_{z_k \in \Delta^{m_k-1}} y_k^\top z_k + S^\tau_k(z_k, x_{-k})$ is computed with $y_k$ instead of $\nabla^k_{x_k}$.
% \begin{align}
%     \hat{\br}_k &= \argmax_{z_k \in \Delta^{m_k-1}} y_k^\top z_k + S^\tau_k(z_k, x_{-k}).
% \end{align}
Likewise, replace all $\nabla^k_{x_k}$ with $y_k$ and $\br_k$ with $\hat{\br}_k$ in equations (\ref{qre_grad}) and (\ref{qre_jac}) when computing the gradient:
% \begin{align}
%     &\nabla_{x_i} \hat{\mathcal{L}}^{\tau}_{adi}(\boldsymbol{x},\boldsymbol{y}) = -(y_i - \tau (\ln(x_i) + 1)) \nonumber
%     \\ &+ \sum_{j \ne i} \Big[ J_{x_i}(\hat{\br}_j)^\top (y_j - \tau (\ln(\hat{\br}_j) + 1)) + H^j_{ij} (\hat{\br}_j - x_j) \Big] \label{qre_grad_aux}
%     \\ &\text{with } J_{x_i}(\hat{\br}_j) = \frac{1}{\tau} (\texttt{diag}(\hat{\br}_j) - \hat{\br}_j \hat{\br}_j^\top) H^j_{ji}. \label{qre_jac_aux}
% \end{align}

\subsection{Putting It All Together}
\label{convergence}
% \label{annealing}
% \ian{table of complexity (scale) and convergence to Nash}
\begin{algorithm}[H]
\begin{algorithmic}[1]
    \STATE Given: Strategy learning rate $\eta_x$, auxiliary learning rate $\eta_y$, initial temperature $\tau$ ($=100$), ADI threshold $\epsilon$, total iterations $T$, simulator $\mathcal{G}_i$ that returns player $i$'s payoff given a joint action.
    \STATE $\boldsymbol{x} \leftarrow \{ \frac{1}{m_i} \boldsymbol{1} \,\, \forall \,\, i\}$
    \STATE $\boldsymbol{y} \leftarrow \{ \boldsymbol{0} \,\, \forall \,\, i \}$
    \FOR{$t = 1: T$}
        \STATE $a_i \sim x_i \,\, \forall \,\, i$ \label{start}
        \FOR{$i \in \{1, \ldots, n\}$}
            \FOR{$j \ne i \in \{1, \ldots, n\}$}
                \STATE $H^i_{ij}[r,c] \leftarrow \mathcal{G}_i(r,c,a_{-ij}) \,\, \forall \,\, r \in \mathcal{A}_i, c \in \mathcal{A}_j$
            \ENDFOR
        \ENDFOR \label{end}
        \STATE $\nabla^i_{x_i} = H^i_{ij} x_j$ for any $x_j$ (or average the result over all $j$)
        \STATE $y_i \leftarrow y_i - \max(\frac{1}{t}, \eta_y) (\nabla^i_{x_i} - y_i)$
        \STATE $x_i \leftarrow x_i - \eta_x \nabla_{x_i} \hat{\mathcal{L}}^{\tau}_{adi}(\boldsymbol{x}, \boldsymbol{y})$ (def. in~\S\ref{amortized_estimates} and code in Appx.~\ref{app:code})
        % \STATE $\hat{\mathcal{L}}^{\tau}_{adi}(x) = \mathcal{L}^{\tau}_{adi}(x)$ with $\nabla^i_{x_i} = y^i$
        \IF{$\hat{\mathcal{L}}^{\tau}_{adi}(\boldsymbol{x}, \boldsymbol{y}) < \epsilon$ (def. in~\eqref{amortized_exp_reg})}
            \STATE $\tau \leftarrow \frac{\tau}{2}$ \label{anneal}
        \ENDIF
    \ENDFOR
    \STATE return $\boldsymbol{x}$
\end{algorithmic}
\caption{ADIDAS}
\label{alg_saped}
\end{algorithm}

Algorithm~\ref{alg_saped}, ADIDAS, is our final algorithm.
% which incorporates an annealing schedule as discussed in~\S\ref{annealing} for the entropy coefficient $\tau$.
% ADIDAS attempts to trace the unique continuum of Nash equilibria of Shannon entropy regularized games (i.e., quantal response equilibria) with temperature decaying from infinity to zero~\citep{mckelvey1995quantal,turocy2005dynamic}\textemdash see Figure~\ref{fig:manynasherror}. McKelvey and Palfrey~\citet{mckelvey1995quantal} call this unique endpoint the \emph{limiting logit equilibrium} and show that the mixed strategies estimated from actual human gameplay lie on or near this unique path for several repeated matrix games. 
ADIDAS attempts to approximate the unique continuum of quantal response equilibria by way of a quasi-stationary process\textemdash see Figure~\ref{fig:homotopy}. Whenever the algorithm finds a joint strategy $\boldsymbol{x}$ exhibiting $\hat{\mathcal{L}}^{\tau}_{adi}$ below a threshold $\epsilon$ for the game regularized with temperature $\tau$, the temperature is exponentially reduced (line~\ref{anneal} of ADIDAS) as suggested in~\citep{turocy2005dynamic}. Incorporating stochastic optimization into the process enables scaling the classical homotopy approach to extremely large games (large payoff tensors). At the same time, the homotopy approach selects a unique limiting equilibrium and, symbiotically, helps alleviate gradient bias, further amortized by the reuse of historical play.

\paragraph{Limitations:} As mentioned earlier, gradient bias precludes a rigorous convergence proof of ADIDAS. However, recent work showed that gradient estimators that are biased, but consistent worked well empirically~\citep{chen2018fastgcn} and follow-up analysis suggests consistency may be an important property~\citep{chen2018stochastic}. Bias is also being explored in the more complex Riemannian optimization setting where it has been proven that the amount of bias in the gradient shifts the stationary point by a proportional amount~\citep{durmus2020convergence}. Note that ADIDAS gradients are also consistent in the limit of infinite samples of joint play, and we also find that biased stochastic gradient descent maintains an adequate level of performance for the purpose of our experiments.

No-regret algorithms scale, but have been proven not to converge to Nash~\citep{flokas2020no} and classical solvers~\citep{mckelvey2014gambit} converge to Nash, but do not scale. ADIDAS suffers from gradient bias, an issue that may be further mitigated by future research. In this sense, ADIDAS is one of the few, if only, algorithms that can practically approximate Nash in many-player, many-action normal-form games.

\begin{figure}
    \centering
    % \includegraphics[width=0.3\textwidth]{figures/ManyNashPathErrorsNoisyShadows.pdf}
    \begin{subfigure}[b]{.49\textwidth}
        \centering
        \includegraphics[width=0.5\textwidth]{figures/ManyNashPathErrorsNoisyShadows.pdf}
        \caption{ADIDAS pathologies \label{fig:manynasherror}}
    \end{subfigure}
    \begin{subfigure}[b]{.49\textwidth}
        \centering
        \includegraphics[width=0.55\textwidth]{figures/el_farol_adi_surface_v3_descent_traj.png}
        \caption{$10$-player, 2-action El Farol homotopy \label{fig:el_farol_homotopy}}
    \end{subfigure}
    % \includegraphics[scale=0.2]{figures/el_farol_adi_surface.png}
    \caption{(\subref{fig:manynasherror}) In the presence of multiple equilibria, ADIDAS may fail to follow the path to the uniquely defined Nash due to gradient noise, gradient bias, and a coarse annealing schedule. If these issues are severe, they can cause the algorithm to get stuck at a local optimum of $\mathcal{L}^{\tau}_{adi}$\textemdash see Figure~\ref{fig:dipmedexp_ate} in \S\ref{large_scale}. (\subref{fig:el_farol_homotopy}) Such concerns are minimal for the El Farol Bar stage game by~\citet{arthur1994complexity}. The solid black curves represent (biased) descent trajectories while the dashed segments indicate the temperature is being annealed.}
    \label{fig:homotopy}
\end{figure}

\begin{table}[ht!]
    \centering
    \begin{tabular}{c|c|c|c}
        Alg Family & Classical & No-Regret & This Work \\ \hline \hline
        Convergence to Nash & Yes & No & Yes$^\dag$ \\ \hline
        Payoffs Queried & $nm^n$ & $Tnm^{\ddag}$ & $T(nm)^2$
    \end{tabular}
    \caption{Comparison of solvers. $^\dag$See \emph{Limitations} in \S\ref{convergence} and Appx.~\ref{app:conv:sto}. $^\ddag$Reduce to $T$ at the expense of higher variance.}
    \label{tab:nealg_comp}
\end{table}
% A game simulator takes as input an action for every player and returns the payoff for a desired player (in line 8 of Alg 1, it returns the payoff for player $i$.

% \begin{figure}
%     \begin{minipage}{0.59\textwidth}
%         \begin{algorithm}[H]
%             \begin{algorithmic}[1]
%                 \STATE Given: Strategy learning rate $\eta_x$, auxiliary learning rate $\eta_y$, initial temperature $\tau$ ($=1$), ADI threshold $\epsilon$, total iterations $T$, game simulator $\mathcal{G}_i$ that returns player $i$'s payoff given a joint action.
%                 \STATE $x \leftarrow \{ \frac{1}{m_i} \boldsymbol{1} \,\, \forall \,\, i\}$
%                 \STATE $y \leftarrow \{ \boldsymbol{0} \,\, \forall \,\, i \}$
%                 \FOR{$t = 1: T$}
%                     \STATE $a_i \sim x_i \,\, \forall \,\, i$ \label{start}
%                     \FOR{$i \in \{1, \ldots, n\}$}
%                         \FOR{$j \ne i \in \{1, \ldots, n\}$}
%                             \STATE $H^i_{ij}[r,c] \leftarrow \mathcal{G}_i(r,c,a_{-ij}) \,\, \forall \,\, r \in \mathcal{A}_i, c \in \mathcal{A}_j$
%                         \ENDFOR
%                     \ENDFOR \label{end}
%                     \STATE $\nabla^i_{x_i} = H^i_{ij} x_j$ for any $x_j$ (or mean over $j$)
%                     \STATE $y_i \leftarrow y_i - \max(\frac{1}{t}, \eta_y) (\nabla^i_{x_i} - y_i)$
%                     \STATE $x_i \leftarrow x_i - \eta_x \nabla_{x_i} \mathcal{L}^{\tau}_{adi}$ (def. in~\S\ref{ped_grads})
%                     % \STATE $\hat{\mathcal{L}}^{\tau}_{adi}(x) = \mathcal{L}^{\tau}_{adi}(x)$ with $\nabla^i_{x_i} = y^i$
%                     \IF{$\hat{\mathcal{L}}^{\tau}_{adi}(\boldsymbol{x}, \boldsymbol{y}) < \epsilon$ (def. in~\eqref{amortized_exp_reg})}
%                         \STATE $\tau \leftarrow \frac{\tau}{2}$ \label{anneal}
%                     \ENDIF
%                 \ENDFOR
%                 \STATE return $\boldsymbol{x}$
%             \end{algorithmic}
%         \caption{ADIDAS}
%         \label{alg_saped}
%         \end{algorithm}
%     \end{minipage}
%     \begin{minipage}{0.39\textwidth}
%         \begin{tabular}{c|c|c}
%             Alg Family & Convergence to NE & Payoffs Queried \\ \hline \hline
%             Classical & Yes & $nm^n$ \\ \hline
%             No-Regret & No & $Tnm$** \\ \hline
%             This Work & Yes* & $T(nm)^2$
%         \end{tabular}
%         \caption{Comparison of solvers. *See \S\ref{convergence} for discussion of convergence. **Can be reduced to $T$ at the expense of higher variance.}
%         \label{tab:nealg_comp}
%     \end{minipage}
% \end{figure}

% \begin{figure}
%     \begin{minipage}{0.69\textwidth}
%         \begin{tabular}{c|c|c|c}
%             Alg Family & Classical & No-Regret & This Work \\ \hline \hline
%             Convergence to Nash & Yes & No & Yes* \\ \hline
%             Payoffs Queried & $nm^n$ & $Tnm$** & $T(nm)^2$
%         \end{tabular}
%         \caption{Comparison of solvers. *See \S\ref{convergence} for discussion of convergence. **Can be reduced to $T$ at the expense of higher variance.}
%         \label{tab:nealg_comp}
%     \end{minipage}
%     \begin{minipage}{0.29\textwidth}
%         \includegraphics[width=\textwidth]{figures/ManyNashPathErrorsNoisyShadows.pdf}
%         \caption{In the presence of multiple equilibria, ADIDAS may fail to follow the path to the uniquely defined Nash due to gradient noise, gradient bias, and a coarse annealing schedule. If the combination of these issues is severe, they can cause the algorithm to get stuck at a local optimum of $\mathcal{L}^{\tau}_{adi}$\textemdash see Appx.~\ref{local_opt}.}
%         \label{fig:manynasherror}
%     \end{minipage}
% \end{figure}

% \textcolor{red}{Update algorithm to include primitive annealing technique. Update expeiriments as well.}

\subsection{Complexity and Savings}
\label{scale}

% \ian{mention blotto example here} \textcolor{red}{the blotto experiments we run are really too small to make a strong point here}

A normal form game may also be represented with a tensor $U$ in which each entry $U[i, a_1, \ldots, a_n]$ specifies the payoff for player $i$ under the joint action $(a_1, \ldots, a_n)$. In order to demonstrate the computational savings of our approach, we evaluate the ratio of the number of entries in $U$ to the number of entries queried (in the sense of~\citep{babichenko2016query,fearnley2015learning,fearnley2016finding}) for computing a single gradient, $\nabla \mathcal{L}^{\tau}_{adi}$. This ratio represents the number of steps that a gradient method can take before it is possible to compute $\mathcal{L}^{\tau}_{adi}$ exactly in expectation.
% We assume evaluating a single entry of the payoff tensor is expensive relative to executing dot products against the tensor. Note that this argument ignores the possibility of evaluating blocks of payoffs in parallel, however, it also ignores the fact that even once the tensor is totally evaluated, computing the true expected deviation incentive still requires solving for the Nash; to be clear, the former weakens our argument while the latter strengthens it.
% As an example of the latter, a true expected gradient costs about $3$ times more than a single stochastic gradient in Blotto($10$ coins, $3$ fields, $4$ players).

Without further assumptions on the game, the number of entries in a general payoff tensor is $nm^n$. In contrast, computing the stochastic deviation incentive gradient requires computing $H_{ij}^j$ for all $i, j$ requiring less than $(nm)^2$ entries\footnote{Recall $\nabla^i_{x_i}$ can be computed with $\nabla^i_{x_i} = H^i_{ij} x_j$ for any $x_j$.}. The resulting ratio is $\frac{1}{n} m^{n-2}$.
%For concreteness, for a Blotto game with $f$ fields and $c$ coins, each player has $m = \frac{(f + c - 1)!}{c! (f - 1)!}$ possible actions.
%
% So for a $3$-player Blotto game with $4$ fields and $10$ coins per player, each player has $66$ actions, and this implies $22$ descent updates for stochastic gradient descent.
%
For a $7$-player, $21$-action game, this implies at least $580,000$ descent updates can be used by stochastic gradient descent.

If the game is symmetric and we desire a symmetric Nash, the payoff tensor can be represented more concisely with $\frac{(m + n - 1)!}{n! (m - 1)!}$ entries (number of multisets of cardinality $n$ with elements taken from a finite set of cardinality $m$). The number of entries required for a stochastic gradient is less than $m^2$. Again, for a $7$-player $21$-action game, this implies at least $2,000$ update steps. Although there are fewer unique entries in a symmetric game, we are not aware of libraries that allow sparse storage of or efficient arithmetic on such permutation-invariant tensors. ADIDAS can exploit this symmetry.

% AlphaStar trained against bots sampled from a population of $600$. The sampling distribution was computed as the Nash of a two-player, symmetric, zero-sum game with $600$ actions per player~\citep{vinyals2019alphastar}. Translating this to a $7$-player game like Diplomacy results in a symmetric payoff tensor with $\mathcal{O}(10^{15})$ unique entries. We do not solve such a large game here, but this suggests solving a game of this size is a realistic challenge for future research.

% \textcolor{red}{Even if you can quickly enumerate the tensor, storing it in memory is expensive. Mention Alphastar Nash league looks at 600 checkpoints. In Dip, that means $\approx 6 \times 10^{15}$ unique payoff entries.}

% \begin{itemize}
%     \item number of entries in symmetric payoff tensor (multisets of cardinality n): $\frac{(m + n - 1)!}{n! (m - 1)!}$
%     \item number of computations to form symmetric stochastic gradient: $m^2$
%     \item for $n=7,m=20$, savings allows about $1600$ sgd iterations
%     \item number of entries in general payoff tensor: $nm^n$
%     \item number of computations to form general stochastic gradient: $(nm)^2$
%     \item for $n=7,m=20$, savings allows about $450,000$ sgd iterations
% \end{itemize}

% Can reduce gradient complexity using additional monte carlo estimation (vr in code); results in O(m) games per step and O(m) grad comp. Could also reduce sampling but leave O(m2) grad comp. Just track each $Hij$ over iterations.

==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/sections/05-experiments.tex <==
\section{Experiments}
\label{exp}

% \ian{summarize results}
We test the performance of ADIDAS empirically on very large games. We begin by considering Colonel Blotto, a deceptively complex challenge domain still under intense research~\citep{behnezhad2017faster,boix2020multiplayer}, implemented in OpenSpiel~\citep{LanctotEtAl2019OpenSpiel}. For reference, both the 3 and 4-player variants we consider are an order of magnitude ($>20\times$) larger than the largest games explored in~\citep{porter2008simple}. We find that no-regret approaches as well as existing methods from Gambit~\citep{mckelvey2014gambit} begin to fail at this scale, whereas ADIDAS performs consistently well. At the same time, we empirically validate our design choice regarding amortizing gradient estimates (\S\ref{amortized_estimates}). Finally, we end with our most challenging experiment, the approximation of a unique Nash of a 7-player, 21-action (> billion outcome) Diplomacy meta-game.

% ADIDAS on Blotto
% with and without y
% with varying # of samples
% legend:
% FTRL
% RM
% QRE-auto w/ y, 1 sample
% QRE-auto w/out y, 1 sample
% QRE-auto w/ y, inf samples

% ADIDAS on Shapleys
% legend:
% FTRL
% RM
% QRE-auto w/ y, 1 sample

% ADIDAS on GAMUT
% legend:
% FTRL
% RM
% QRE-auto w/ y, 1 sample
% QRE-auto w/ y, 100 samples
% QRE-auto w/ y, inf samples

% We first empirically validate our design choices regarding the effect of an entropy bonus on loss and gradient bias (\S\ref{bias_intuition}+\S\ref{ped_grads}), scaling to large games (\S\ref{scale}), amortizing gradient estimates (\S\ref{amortized_estimates}), and annealing (\S\ref{annealing}). We use $3$ and $4$-player variants of Colonel Blotto, a deceptively complex challenge domain still currently under intense research~\citep{boix2020multiplayer}, implemented in OpenSpiel~\citep{LanctotEtAl2019OpenSpiel} to expose the effects of our choices. For reference, the 4 player game is an order of magnitude ($24\times$) larger than the largest explored in~\citep{porter2008simple} and already pushes the limits of the classical solvers available in Gambit~\citep{mckelvey2014gambit}. We then demonstrate our approach, which incrementally accesses the payoff tensor through samples, on solving games relevant to Diplomacy that are three orders of magnitude larger ($4034\times$) than those in~\citep{porter2008simple}. The conclusion is that ADIDAS can practically approximate Nash in large games where previous algorithms are unsuitable.

% Blotto (3 player, 286 action) 22x (8p, 5a)
% Blotto (4 player, 66 action) 24x (8p, 5a)
% Diplomacy (7 player, 21 action) 4000x (8p, 5a)

% Porter et al explores games (players, actions)
% (8 player, 5 action) 3,125,000
% (6 player, 8 action) 1,572,864

% We do not presume this algorithm achieves optimal convergence rates or is guaranteed to converge to a Nash. We are more interested in making the current intractable problem of approximating Nash in large normal form games, tractable. With that said, ADIDAS 
% We expect this to be a fruitful area for further research.

% We use the following notation to indicate variants of the algorithms compared in Table~\ref{tab:competingalgs}. A $y$ superscript prefix, e.g., $^y$\texttt{QRE}, indicates the estimates of payoff gradients are amortized using using historical play; likewise, a $y$$-$$poly$ superscript prefix denotes a variant of the algorithm where the auxiliary variable $y_{ij}$ tracks a running estimate of each $H^i_{ij}$. $\bar{x}_t$ indicates that the average deviation incentive reported is for the average of $\boldsymbol{x}_t$ over learning. A subscript of ${\infty}$ indicates best responses are computed with respect to the true expected payoff gradient (infinite samples). A superscript indicates the temperature of the regularizer, e.g., \texttt{QRE}$^{0.1}$ uses $\tau=0.1$ and \texttt{QRE}$^{auto}$ anneals $\tau$. An $s$ in parentheses indicates lines~\ref{start} to~\ref{end} of ADIDAS are repeated $s$ times, and the resulting $H^i_{ij}$'s are averaged for a more accurate estimate. All runs are performed on virtual Google CPUs (GCUs).
We use the following notation to indicate variants of the algorithms compared in Table~\ref{tab:competingalgs}. A $y$ superscript prefix, e.g., $^y$\texttt{QRE}, indicates the estimates of payoff gradients are amortized using historical play; its absence indicates that a fresh estimate is used instead. $\bar{x}_t$ indicates that the average deviation incentive reported is for the average of $\boldsymbol{x}^{(t)}$ over learning. A subscript of ${\infty}$ indicates best responses are computed with respect to the true expected payoff gradient (infinite samples). A superscript $auto$ indicates the temperature $\tau$ is annealed according to line~\ref{anneal} of~\Algref{alg_saped}. An $s$ in parentheses indicates lines~\ref{start}-\ref{end} of ADIDAS are repeated $s$ times, and the resulting $H^i_{ij}$'s are averaged for a more accurate estimate. Each game is solved on 1 CPU, except Diplomacy (see Appx.~\ref{app:runtime}).

\begin{table}[ht!]
    \begin{tabular}{l|l}
        \texttt{FTRL} & Simultaneous Gradient Ascent \\
        \texttt{RM} & Regret-Matching~\citep{blackwell1956analog} \\
        % \texttt{PED} & ADIDAS with no entropy or $y$ \\
        \texttt{ATE} & ADIDAS with Tsallis (Appx.~\ref{ate_exp}) \\
        \texttt{QRE} & ADIDAS with Shannon
    \end{tabular}
    \caption{Algorithms}
    \label{tab:competingalgs}
\end{table}
\vspace{-3em}
\begin{table}[ht!]
    \begin{tabular}{r|l}
        $\eta_x$ & $10^{-5}, 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}$ \\
        $\eta_x^{-1} \cdot \eta_y$ & $1, 10, 100$ \\
        $\tau$ & $0.0, 0.01, 0.05, 0.10$ \\
        $\Pi_{\Delta}(\nabla \mathcal{L}_{adi})$ & Boolean \\
        Bregman-$\psi(\boldsymbol{x})$ & $\{\frac{1}{2}||\boldsymbol{x}||^2, -\mathcal{H}(\boldsymbol{x})\}$ \\
        $\epsilon$ & $0.01, 0.05$
    \end{tabular}
    \caption{Hyperparameter Sweeps}
    \label{tab:hypsweeps}
\end{table}

% % \textcolor{red}{Table of competing methods.}
% \begin{table}[ht!]
%     \centering
%     \begin{tabular}{r|l}
%         \texttt{FTRL} & Simultaneous Gradient Ascent \\
%         \texttt{RM} & Regret-Matching~\citep{blackwell1956analog} \\
%         \texttt{PED} & ADIDAS with no regularization or $y$ \\
%         \texttt{ATE} & ADIDAS with Tsallis regularization (Appendix~\ref{ate_exp}) \\
%         \texttt{QRE} & ADIDAS with Shannon regularization
%     \end{tabular}
%     \caption{Algorithms}
%     \label{tab:competingalgs}
% \end{table}
% % RM: hart2000simple

Sweeps are conducted over whether to project gradients onto the simplex ($\Pi_{\Delta}(\nabla \mathcal{L}_{adi})$), whether to use a Euclidean projection or entropic mirror descent~\citep{beck2003mirror} to constrain iterates to the simplex, and over learning rates. Averages over $10$ runs of the best hyperparameters are then presented\footnote{Best hyperparameters are used because we expect running ADIDAS with multiple hyperparameter settings in parallel to be a pragmatic approach to approximating Nash.} except for Diplomacy for which we present all settings attempted (more in Appx.~\ref{app:more_dip}). Performance is measured by $\mathcal{L}_{adi}$, a.k.a. \texttt{NashConv}~\citep{lanctot2017unified}. For symmetric games, we enforce searching for a symmetric equilibrium (see Appx.~\ref{app:sym}).

% \ian{explain why certain baselines are missing. avoid clutter. fair comparisons. etc}
For sake of exposition, we do not present all baselines in all plots, however, we include the full suite of comparisons in the appendix. Our experiments demonstrate that without any additional prior information on the game, ADIDAS is the only practical approach for approximating a Nash equilibrium over many-players and many-actions. We argue this by systematically ruling out other approaches on a range of domains. For example, in Figure~\ref{fig:blotto_tracking_qre}, \texttt{RM} reduces ADI adequately in Blotto. We do not present \texttt{RM} with improvements in Figure~\ref{fig:blotto_tracking_qre} such as using exact expectations, \texttt{RM}$_{\infty}$, or averaging its iterates, \texttt{RM}$(\bar{x}_t)$, because we show that both these fail to save \texttt{RM} on the GAMUT game in Figure~\ref{fig:noregfail}. In other words, we do not present baselines that are unnecessary for logically supporting the claim above. Code is available at \href{https://github.com/deepmind/open_spiel}{github.com/deepmind/open\_spiel}~\cite{LanctotEtAl2019OpenSpiel}.

% \begin{table}[ht!]
%     \centering
%     \begin{tabular}{r|l}
%         $\eta_x$ & $10^{-5}, 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}$ \\
%         $\eta_x^{-1} \cdot \eta_y$ & $1, 10, 100$ \\
%         $\tau$ & $0.0, 0.01, 0.05, 0.10$ \\
%         $\Pi_{\Delta}(\nabla \mathcal{L}_{adi})$ & Boolean \\
%         $\{\frac{1}{2}||x||^2, -\mathcal{H}(x)\}$ & Bregman-like distance $\psi(x)$ \\
%         $\epsilon$ & $0.01, 0.05$
%     \end{tabular}
%     \caption{Hyperparameter Sweeps}
%     \label{tab:hypsweeps}
% \end{table}

% \paragraph{Bias re. \S\ref{bias_intuition}+\S\ref{ped_grads}} We first empirically verify that adding an entropy regularizer to the utilities introduces a trade-off: too little and the best-response operator will have high bias; too much and risk solving for the Nash of a game we are not interested in. Figure~\ref{fig:gradient_bias_qre} in the appendix supports that there exists a sweet spot in the middle for moderate amounts of regularization (temperatures).

% In Figure~\ref{fig:blotto_tracking_qre}, we also see a more general relationship between temperature and convergence rate. Higher temperatures appear to result in faster initial convergence ($\mathcal{L}_{adi}$ spikes initially in Figure~\ref{fig:blotto3track_qre} for $\tau<0.1$) and lower variance but higher asymptotes, while the opposite holds for lower temperatures. These results suggest annealing the temperature over time to achieve fast initial convergence and lower asymptotes. Lower variance should also be possible by carefully annealing the learning rate to allow $y$ to accurately perform tracking. Fixed learning rates were used here; we leave investigating learning rate schedules to future work.

% Figure~\ref{fig:blotto4track_qre} shows higher temperatures (through a reduction in gradient bias) can result in accelerated convergence.

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{.4\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/blotto_10_4_3_qre_adi_v2.png}
    \caption{3-player, 286-action Blotto \label{fig:blotto3track_qre}}
    \end{subfigure}
    \begin{subfigure}[b]{.4\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/blotto_10_3_4_qre_adi_v2.png}
    \caption{4-player, 66-action Blotto \label{fig:blotto4track_qre}}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Amortizing estimates of joint play using $\boldsymbol{y}$ can reduce gradient bias, further improving performance (e.g., compare \texttt{QRE}$^{auto}$ to $^y$\texttt{QRE}$^{auto}$ in (\subref{fig:blotto3track_qre}) or (\subref{fig:blotto4track_qre})).}
    \label{fig:blotto_tracking_qre}
\end{figure}

% \paragraph{Med-Scale re. \S\ref{scale}} 
\subsection{Med-Scale re. \S\ref{scale}}
\label{med_scale}
Govindan-Wilson is considered a state-of-the-art Nash solver, but it does not scale well to large games. For example, on a symmetric, $4$-player Blotto game with $66$ actions ($10$ coins, $3$ fields), GW, as implemented in Gambit, is estimated to take 53,000 hours\footnote{Public correspondence with primary \texttt{gambit} developer [\href{https://github.com/gambitproject/gambit/issues/261\#issuecomment-660894391}{link}].}. Of the solvers implemented in Gambit, none finds a symmetric Nash equilibrium within an hour\footnote{\texttt{gambit-enumpoly} returns several non-symmetric, pure Nash equilibria. Solvers listed in Appx.~\ref{app:gambit_solvers}. Symmetric equilibria are necessary for ranking in symmetric meta-games.}. Of those, \texttt{gambit-logit}~\citep{turocy2005dynamic} is expected to scale most gracefully. Experiments from the original paper are run on maximum $5$-player games ($2$-actions per player) and $20$-action games ($2$-players), so the $4$-player, $66$-action game is well outside the original design scope. Attempting to run $\texttt{gambit-logit}$ anyways with a temperature $\tau=1$ returns an approximate Nash with $\mathcal{L}_{adi}=0.066$ after $101$ minutes. In contrast, Figure~\ref{fig:blotto4track_qre} shows ADIDAS achieves a lower ADI in $\approx 3$ minutes.
% already cited earlier: ~\citep{mckelvey2014gambit}
% (approx 53k hrs for blotto problem - \url{https://github.com/gambitproject/gambit/issues/261#issuecomment-660894391})

% Gambit solvers - none appear fit to run on very large games. gambit-logit~\citep{turocy2005dynamic} is best prepared, but even in the paper, max player is 5 (5,2) and max actions is 20 (2,20). gambit-logit still takes forever (gambit-logit lambda=1.02 qre solution after 101minutes with nash-conv = 0.0656848861190602)

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{.45\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/mod_shapleys_qre_adi_v2.png}
    \caption{2-player, 3-action modified Shapley's \label{fig:modshapley_qre}}
    \end{subfigure}
    \begin{subfigure}[b]{.45\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/gamut_d7_qre_adi_v2.png}
    \caption{6-player, 5-action GAMUT-D7 \label{fig:gamutd7_qre}}
    \end{subfigure}
    \vspace{-5pt}
    \caption{ADIDAS reduces $\mathcal{L}_{adi}$ in both these nonsymmetric games. In contrast, regret matching stalls or diverges in game~(\subref{fig:modshapley_qre}) and diverges in game~(\subref{fig:gamutd7_qre}). \texttt{FTRL} makes progress in game~(\subref{fig:modshapley_qre}) but stalls in game~(\subref{fig:gamutd7_qre}). In game~(\subref{fig:modshapley_qre}), created by~\protect\citet{ostrovski2013payoff}, to better test performance, $\boldsymbol{x}$ is initialized randomly rather than with the uniform distribution because the Nash is at uniform.}
    \label{fig:noregfail}
\end{figure}

\paragraph{Auxiliary $y$ re. \S\ref{amortized_estimates}} The introduction of auxiliary variables $y_i$ are supported by the results in Figure~\ref{fig:blotto_tracking_qre}\textemdash $^y$\texttt{QRE}$^{auto}$ significantly improves performance over \texttt{QRE}$^{auto}$ and with low algorithmic cost.

% \paragraph{Annealing $\tau$ re. \S\ref{annealing}} ADIDAS includes temperature annealing, replacing the need to preset $\tau$ with instead an ADI threshold $\epsilon$. Figure~\ref{fig:blotto_qre} compares this approach against other variants of the algorithm and shows this automated annealing mechanism reaches comparable final levels of ADI.

% \begin{figure}[!ht]
%     \centering
%     \begin{subfigure}[b]{.4\textwidth}
%     \includegraphics[width=\textwidth]{figures/blotto_10_4_3_qre_adi.png}
%     \caption{3-player Blotto \label{fig:blotto3_qre}}
%     \end{subfigure}
%     \begin{subfigure}[b]{.4\textwidth}
%     \includegraphics[width=\textwidth]{figures/blotto_10_3_4_qre_adi.png}
%     \caption{4-player Blotto \label{fig:blotto4_qre}}
%     \end{subfigure}
%     % \begin{subfigure}[b]{.49\textwidth}
%     % \includegraphics[width=\textwidth]{figures/diplomacy_delta_4.pdf}
%     % \caption{Diplomacy \label{fig:diplomacy}}
%     % \end{subfigure}
%     \vspace{-5pt}
%     \caption{Average deviation incentive of the symmetric joint strategy $\boldsymbol{x}^{(t)}$ is plotted against algorithm iteration $t$. Despite \texttt{FTRL}'s lack of convergence guarantees, it converges quickly in these games.}
%     % (\subref{fig:diplomacy}) Similar qualitative results hold for normal form games constructed from subsampled turns in a Diplomacy match.
%     \label{fig:blotto_qre}
%     % $\mathcal{O}(m)$ trajectories are noisier than $\mathcal{O}(m^2)$ variants (at least for \texttt{qre}) as expected, but they are still effective.
% \end{figure}

% We originally planned to run experiments on Blotto and the meta-game of Diplomacy ($7$-players, $5$-actions per player). Unfortunately, each of these games turned out to be quite transitive which means policy gradient converges very quickly obviating the need for a more sophisticated approach like SAPED.

\paragraph{No-regret, No-convergence re.~\S\ref{convergence}} In Figure~\ref{fig:blotto_tracking_qre}, \texttt{FTRL} and \texttt{RM} achieve low ADI quickly in some cases. \texttt{FTRL} has recently been proven not to converge to Nash, and this is suggested to be true of no-regret algorithms in general~\citep{flokas2020no,mertikopoulos2018cycles}. Before proceeding, we demonstrate empirically in Figure~\ref{fig:noregfail} that \texttt{FTRL} and \texttt{RM} fail on games where ADIDAS significantly reduces ADI. Note that GAMUT (D7) was highlighted as a particularly challenging problem for Nash solvers in~\citep{porter2008simple}.
% \textcolor{red}{Add modified Shapley's and D7}.

% However, in some cases, SAPED can outperform policy gradient, such as Blotto($10$ coins, $3$ fields, $4$ players).

% Figures~\ref{fig:diplomacy} and~\ref{fig:dipsub} run a comparison on two Diplomacy meta-games and $40$ subsampled tensors taken from the $40$ turns of a single Diplomacy match.
% Figure~\ref{fig:diplomacy} runs a comparison on two Diplomacy meta-games.

% \begin{figure}[!ht]
%     \centering
%     \begin{subfigure}[b]{.225\textwidth}
%     \includegraphics[width=\textwidth]{figures/dip_fp.pdf}
%     \caption{Diplomacy FP \label{fig:dipfp}}
%     \end{subfigure}
%     \begin{subfigure}[b]{.225\textwidth}
%     \includegraphics[width=\textwidth]{figures/dip_ibr.pdf}
%     \caption{Diplomacy IBR \label{fig:dipibr}}
%     \end{subfigure}
%     \vspace{-5pt}
%     \caption{(\subref{fig:dipfp}) FP; (\subref{fig:dipibr}) IBR. The maximum a single agent can exploit the symmetric joint strategy $\boldsymbol{x}^{(t)}$ is plotted against algorithm iteration $t$. Many of the algorithms quickly achieve near zero $\mathcal{L}_{adi}$, so unlike in the other experiments, hyperparameters are selected according according to the earliest point at which exploitablity falls below $0.01$ with ties split according to the final value.}
%     % (\subref{fig:diplomacy}) Similar qualitative results hold for normal form games constructed from subsampled turns in a Diplomacy match.
%     \label{fig:diplomacy}
%     % $\mathcal{O}(m)$ trajectories are noisier than $\mathcal{O}(m^2)$ variants (at least for \texttt{qre}) as expected, but they are still effective.
% \end{figure}


% \paragraph{Estimating Exploitability from Historical Play}
% So far, we have compared scalable Nash solvers in settings where we can actually compute ADI using true expectations, however, in very large scale settings where the payoff tensor cannot be enumerated, this is not possible. Therefore, we must estimate the ADI. Figure~\ref{fig:exp_est} shows how the estimates of deviation incentive computed from historical play track their true expected value throughout training.

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{.45\textwidth}
    \centering
    \includegraphics[width=0.75\textwidth]{figures/dipmednash_adi.pdf}
    \caption{7-player, 5-action symmetric Nash ($x_t$) \label{fig:dipmednash_ate}}
    \end{subfigure}
    \begin{subfigure}[b]{.45\textwidth}
    \centering
    \includegraphics[width=0.75\textwidth]{figures/dipmedexp_adi.pdf}
    \caption{ADI Estimate \label{fig:dipmedexp_ate}}
    \end{subfigure}
    \vspace{-5pt}
    \caption{(\subref{fig:dipmednash_ate}) Evolution of the symmetric Nash approximation returned by ADIDAS for the $7$-player Diplomacy meta-game that considers a subset $\{0, 2, 4, 10, 20\}$ of the available $21$ bots; (\subref{fig:dipmedexp_ate}) ADI estimated from auxiliary variable $\boldsymbol{y}_t$. Black vertical lines indicate the temperature $\tau$ was annealed.}
    %  (line~\ref{anneal} of Algorithm~\ref{alg_saped}). 
    \label{fig:diplomacy_med_ate}
\end{figure}

% \paragraph{Large-Scale}
\subsection{Large-Scale}
\label{large_scale}
Figure~\ref{fig:diplomacy_med_ate} demonstrates an empirical game theoretic analysis~\citep{wellman2006methods,jordan2007empirical,wah2016empirical} of a large symmetric $7$-player Diplomacy meta-game where each player elects $1$ of $5$ trained bots to play on their behalf. Each bot represents a snapshot taken from an RL training run on Diplomacy~\citep{anthony2020learning}. In this case, the expected value of each entry in the payoff tensor represents a winrate. Each entry can only be estimated by simulating game play, and the result of each game is a Bernoulli random variable (ruling out deterministic approaches, e.g., \texttt{gambit}). To estimate winrate within $0.01$ (ADI within $0.02$) of the true estimate with probability $95\%$, a Chebyshev bound implies more than $223$ samples are needed. The symmetric payoff tensor contains $330$ unique entries, requiring over $73$ thousand games in total. ADIDAS achieves near zero ADI in less than $7$ thousand iterations with $50$ samples of joint play per iteration ($\approx 5 \times$ the size of the tensor).
%
% Hoeffding
% \begin{align}
%     P(\vert S_n - E_n \vert > t) &< 2 \texttt{adi}\big( \frac{-2t^2}{nC^2} \big)
%     \\ C = (1 - 0) / n
%     \\ P(\vert \sum_{i=1}^n \frac{x_i}{n} - \sum_{i=1}^n \frac{\mathbb{E}[x_i]}{n} \vert > t) &< 2 \texttt{adi}\big( -2nt^2 \big)
%     \\ P(\vert \bar{x} - \mathbb{E}[x_i] \vert > t) &< 2 \texttt{adi}\big( -2nt^2 \big) \le 0.05
%     \\ n = \frac{\ln(\frac{2}{0.05})}{2t^2} &> 18000 \text{ for } t=0.01
% \end{align}
%
% Chebyshev
% Var(Bernoulli) <= pq = p(1-p) <= 1/4
% Var(Mean Bernoullis) <= 1/4 * 1/n^2
% P(\vert \bar{x} - \mathbb{E}[x_i] \vert > t) &< Var(Mean Bern) / t^2 = 1/(4n^2t^2) \le 0.05
%     \\ n = 1/(2t * sqrt(0.05)) &> 223 \text{ for } t=0.01
% 223 * 330 = 73590
% 223 * 888030 = 198030690
%
% 2t * sqrt(0.5) = 1/n
% t = 1 /(2 * sqrt(0.5) * n)
%
\paragraph{Continuum of QREs approaching LLE}
The purpose of this work is to approximate a unique Nash (the LLE) which ADIDAS is designed to do, however, the approach ADIDAS takes of attempting to track the continuum of QREs (or the continuum defined by the Tsallis entropy) allows returning these intermediate QRE strategies which may be of interest. Access to these intermediate approximations can be useful when a game playing program cannot wait for ADIDAS's final output to play a strategy, for example, in online play. Interestingly, human play appears to track the continuum of QREs in some cases where the human must both learn about the game (rules, payoffs, etc.) whilst also evolving their strategy~\citep{mckelvey1995quantal}.
\balance
Notice in Figure~\ref{fig:diplomacy_med_ate} that the trajectory of the Nash approximation is not monotonic; for example, see the kink around $2000$ iterations where bots $10$ and $20$ swap rank. The continuum of QRE's from $\tau=\infty$ to $\tau=0$ is known to be complex providing further reason to carefully estimate ADI and its gradients.

% \subsubsection{Convergence to a Local Optimum: Example}
% \label{local_opt}
\paragraph{Convergence to a Local Optimum}
\balance
One can also see from Figure~\ref{fig:dipmedexp_ate} that $^y\texttt{ATE}^{0.0}$ has converged to a suboptimal local minimum in the energy landscape. This is likely due to the instability and bias in the gradients computed without any entropy bonus; notice the erratic behavior of its ADI within the first $2000$ iterations.

% \subsection{Convergence to local optimum}
% \label{local_opt}
% \ian{Discussion?}

% \begin{figure}[!ht]
%     \centering
%     \begin{subfigure}[b]{.49\textwidth}
%     \includegraphics[width=\textwidth]{figures/dipbignash_localopt.pdf}
%     \caption{Symmetric Nash ($x_t$) \label{fig:dipbignash_localopt}}
%     \end{subfigure}
%     \begin{subfigure}[b]{.49\textwidth}
%     \includegraphics[width=\textwidth]{figures/dipbigexp_localopt.pdf}
%     \caption{Exploitability Estimate \label{fig:dipbigexp_localopt}}
%     \end{subfigure}
%     \vspace{-5pt}
%     \caption{(\subref{fig:dipbignash_localopt}) Symmetric Nash as a transposed histogram over iterations; (\subref{fig:dipbigexp_localopt}) Deviation incentive estimated from auxiliary variable $y_t$. Black vertical lines indicate the temperature $\tau$ was annealed (line~\ref{anneal} of Algorithm~\ref{alg_saped}).}
%     \label{fig:diplomacy_big_localopt}
% \end{figure}

% \subsubsection{Importance of Entropy Bonus}
% \label{bignash_all}

% \paragraph{Very Large-Scale re. \S\ref{scale}}
\subsection{Very Large-Scale re. \S\ref{scale}}
\label{very_large_scale}
% Computing ADI exactly requires the full payoff tensor, so in very large games, we must estimate ADI. Figure~\ref{fig:exp_est_qre} in the appendix shows how estimates of $\mathcal{L}_{adi}$ computed from historical play track their true expected value throughout training.
%
% Finally, we perform an empirical game theoretic analysis~\citep{wellman2006methods,jordan2007empirical,wah2016empirical} of a large symmetric $7$-player Diplomacy meta-game where each player elects $1$ of $21$ trained bots to play on their behalf. Each bot represents a snapshot taken from an RL training run on Diplomacy~\citep{anthony2020learning}. In this case, the expected value of each entry in the payoff tensor is a winrate. Each entry can only be estimated by simulating game play, and the result of each game is a Bernoulli random variable (ruling out deterministic approaches, e.g., \texttt{gambit}).
Finally, we repeat the above analysis with all $21$ bots.
To estimate winrate within $0.015$ (ADI within $0.03$) of the true estimate with probability $95\%$, a Chebyshev bound implies approximately $150$ samples are needed. The symmetric payoff tensor contains $888,030$ unique entries, requiring over $100$ million games in total. Note that ignoring the symmetry would require simulating $150 \times 21^7 \approx 270$ billion games and computing over a trillion payoffs ($\times7$ players). Simulating all games, as we show, is unnecessarily wasteful, and just storing the entire payoff tensor in memory, let alone computing with it would be prohibitive without special permutation-invariant data structures ($\approx 50$GB with \texttt{float32}). In Figure~\ref{fig:dipbignash_all_ate}, ADIDAS with $\eta_x = \eta_y = 0.1$ and $\epsilon = 0.001$ achieves a stable ADI below $0.03$ in less than $100$ iterations with $10$ samples of joint play per iteration and each game repeated $7$ times ($< 2.5\%$ of the games run by the naive alternative).
% Appx.~\ref{app:more_dip} expands Figure~\ref{fig:dipbignash_ate} with additional data revealing the importance of anealing $\tau$.
As expected, bots later in training (darker lines) have higher mass under the Nash distribution computed by $^y\texttt{ATE}^{auto}$. Runtime is discussed in Appx.~\ref{app:runtime}.
% \ian{waiting for results of experiment with 21 actions and 2 orders magnitude fewer games than naive approach.}

\paragraph{Importance of Entropy Bonus}

Figure~\ref{fig:dipbignash_all_ate} shows how the automated annealing mechanism ($^y\texttt{ATE}^{auto}$) seeks to maintain entropy regularization near a ``sweet spot" \textemdash too little entropy ($^y\texttt{ATE}^{0.0}$) results in an erratic evolution of the Nash approximation and too much entropy ($^y\texttt{ATE}^{1.0}$) prevents significant movement from the initial uniform distribution. Figure~\ref{fig:dipbigexp_ate2} shows that ADIDAS with the automated annealing mechanism meant to trace the QRE continuum achieves a lower ADI than its fixed temperature variants.

% Hoeffding
% \begin{align}
%     P(\vert S_n - E_n \vert > t) &< 2 \texttt{exp}\big( \frac{-2t^2}{nC^2} \big)
%     \\ C = (1 - 0) / n
%     \\ P(\vert \sum_{i=1}^n \frac{x_i}{n} - \sum_{i=1}^n \frac{\mathbb{E}[x_i]}{n} \vert > t) &< 2 \texttt{exp}\big( -2nt^2 \big)
%     \\ P(\vert \bar{x} - \mathbb{E}[x_i] \vert > t) &< 2 \texttt{exp}\big( -2nt^2 \big) \le 0.05
%     \\ n = \frac{\ln(\frac{2}{0.05})}{2t^2} &> 18000 \text{ for } t=0.01
% \end{align}

% Chebyshev
% Var(Bernoulli) <= pq = p(1-p) <= 1/4
% Var(Mean Bernoullis) <= 1/4 * 1/n^2
% P(\vert \bar{x} - \mathbb{E}[x_i] \vert > t) &< Var(Mean Bern) / t^2 = 1/(4n^2t^2) \le 0.05
%     \\ n = 1/(2t * sqrt(0.05)) &> 223 \text{ for } t=0.01
% 223 * 330 = 73590
% 223 * 888030 = 198030690

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{.49\textwidth}
    \centering
    \includegraphics[width=0.75\textwidth]{figures/dipbignash_timeseries_all.pdf}
    \caption{7-player, 21-action symmetric Nash ($x_t$) \label{fig:dipbignash_all_ate}}
    \end{subfigure}
    \begin{subfigure}[b]{.49\textwidth}
    \centering
    \includegraphics[width=0.75\textwidth]{figures/dipbigexp_adi.pdf}
    \caption{ADI Estimate \label{fig:dipbigexp_ate2}}
    \end{subfigure}
    \vspace{-5pt}
    \caption{(\subref{fig:dipbignash_all_ate}) Evolution of the symmetric Nash approximation returned by ADIDAS for the $7$-player, $21$-bot Diplomacy meta-game; (\subref{fig:dipbigexp_ate2}) ADI estimated from auxiliary variable $y_t$. Black vertical lines indicate the temperature $\tau$ was annealed.}
    %  (line~\ref{anneal} of Algorithm~\ref{alg_saped}). 
    % \label{fig:diplomacy_big_all_ate}
    \label{fig:diplomacy_big_ate}
\end{figure}

% \begin{figure}[!ht]
%     \centering
%     \begin{subfigure}[b]{.45\textwidth}
%     \includegraphics[width=\textwidth]{figures/dipbignash_timeseries.pdf}
%     \caption{7-player, 21-action symmetric Nash ($x_t$) \label{fig:dipbignash_ate}}
%     \end{subfigure}
%     \begin{subfigure}[b]{.45\textwidth}
%     \includegraphics[width=\textwidth]{figures/dipbigexp_adi.pdf}
%     \caption{ADI estimate \label{fig:dipbigexp_ate}}
%     \end{subfigure}
%     \vspace{-5pt}
%     \caption{(\subref{fig:dipbignash_ate}) Evolution of the symmetric Nash approximation returned by ADIDAS for the $7$-player, $21$-bot Diplomacy meta-game; (\subref{fig:dipbigexp_ate}) ADI estimated from auxiliary variable $y_t$. Black vertical lines indicate the temperature $\tau$ was annealed.}
%     % Symmetric Nash as a stacked histogram by temperature
%     %  (line~\ref{anneal} of Algorithm~\ref{alg_saped}). 
%     \label{fig:diplomacy_big_ate}
% \end{figure}
% $\eta_x = \eta_y = 1e-1, \epsilon = 1e-3$

In the appendix, we perform additional ablation studies (e.g., no entropy, annealing), measure accuracy of $\hat{\mathcal{L}}^{\tau}_{adi}$, compare against more algorithms on other domains, and consider Tsallis entropy.

% \section{Discussion}
% ADIDAS significantly reduces ADI in several domains: Blotto, a modified Shapley's game, GAMUT's Covariant Game (D7), and a Diplomacy meta-game. However, a large performance gap still exists between this stochastic algorithm and gradient descent on the true expected $\mathcal{L}_{adi}$ (\texttt{PED}$_{\infty}$ in \textbf{black}). Figure~\ref{fig:gamutd7_qre} shows that increasing the number of samples can improve performance, but this means additional computation. While the no-regret algorithms, \texttt{RM} and \texttt{FTRL}, fail in Figure~\ref{fig:noregfail}, they are able to more efficiently solve Blotto.
% We show how the complexity of Algorithm~\ref{alg_saped} can be reduced from $\mathcal{O}(m^2)$ to $\mathcal{O}(m)$, but at the expense of added estimation error.

% The ability to monitor an estimate of performance such as $\mathcal{L}_{adi}$ is important for determining when ADIDAS can be terminated. Therefore, improving the accuracy of the estimates of $\mathcal{L}_{adi}$ and $\nabla_{x} \mathcal{L}_{adi}$ is important.

==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/sections/06-theory.tex <==
% \section{Convergence}
% The continuum of Nash equilibria of entropy regularized games with temperature decaying from infinity to zero defines a unique path to a Nash equilibrium of the original game~\cite{mckelvey1995quantal,turocy2005dynamic}. Our algorithm attempts to roughly approximate this path.

==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}.
  \item Did you describe the limitations of your work?
    \answerYes{} Summarized succinctly in Figure~\ref{fig:manynasherror}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}. We see no obvious negative impact.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}.
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}. See Appendix~\ref{app:conv}.
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}. See Appendix~\ref{app:conv}.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}. We include pseudocode and two key methods in python in the appendix. All games are available via open source libraries (OpenSpiel, gambit, and GAMUT) or referenced directly in papers (e.g., modified Shapley's game).
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}. We report standard error of the mean.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}. See \S\ref{exp} and Appx.~\ref{app:runtime}.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}.
  \item Did you mention the license of the assets?
    \answerNo{}. The OpenSpiel (\href{https://github.com/deepmind/open_spiel/blob/master/LICENSE}{Apache}), gambit (\href{http://www.gambit-project.org/gambit13/index.html}{GNU license}), and GAMUT (\href{http://gamut.stanford.edu/}{Apache license on download page}) licenses are clearly stated on their websites.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}.
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Average Deviation Incentive Descent with Adaptive Sampling (ADIDAS) [arXiv]/sections/conclusion.tex <==
\section{Conclusion}

Existing algorithms either converge to Nash, but do not scale to large games or scale to large games, but do not converge to Nash. We proposed an algorithm to fill this void that queries necessary payoffs through sampling, obviating storing the full payoff tensor in memory. ADIDAS is principled and shown empirically to approximate Nash in large-normal form games.

% Deviation incentive suffers from bias when computed using samples of joint play. Carefully regularizing player utilities with entropy and amortizing estimates using historical play can reduce the effects of bias. Our proposed algorithm is able to iteratively improve an approximation to a Nash distribution without accessing the entire payoff tensor, rendering it scalable to large games where classical solvers fail to return an answer.

% SAPED can be slower than policy gradient in transitive games or games with low support. We leave detecting such settings and selecting the appropriate solver to future work. So far, we have only empirically tested the symmetric solver.

% We will require non-symmetric solvers for subsampled games in Diplomacy. If the associated payoff tensor is small enough, it makes sense to store the utilities from historical play and update their estimates (for noisy values) as new estimates are obtained.

% \subsection{TODO}

% \begin{enumerate}
%     \item Track number of unique joint actions sampled.
%     \item Small-Scale
%     \begin{enumerate}
%         \item Random GAMUT~\citep{nudelman2004run} Sweep (as in Simple Search Methods) with ``solved" condition is when nash-conv drops below 5\% \& 1\% of payoff range. Run gambit-logit, gambit-gnm, and gambit-simpdiv, gambit-ipa plus both deterministic and stochastic variants of nash-conv descent. \textbf{Have really been comparing against D7, not D6.}~\citep{rinott2000number}. Need to write your own version for $\rho \ge 0$. Keep a dict of the joint actions played an their payoff vectors.
%         \item Blotto, Goofspiel, Multi-Sumo. too big for gambit, but run deterministic and stochastic variants of nash-conv with ADI over iterations
%         \item Shapley's game to rule out convergence to Nash of average empirical play of no-regret learners
%         \item Same but for Diplomacy subsampled games with ADI over iterations [Done]
%     \end{enumerate}
%     \item Large-Scale - only stochastic nash-conv descent, only stochastic ADI
%     \begin{enumerate}
%         \item Large Blotto, Goofspiel, Multi-Sumo
%         \item Diplomacy meta-game, lemonade game
%     \end{enumerate}
% \end{enumerate}

% \textcolor{red}{Not aware of special hardware or software for computations with permutation invariant tensors.}

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}.
  \item Did you describe the limitations of your work?
    \answerYes{} Summarized succinctly in Figure~\ref{fig:manynasherror}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}. We see no obvious negative impact.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}.
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}. See Appendix~\ref{app:conv}.
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}. See Appendix~\ref{app:conv}.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}. We include pseudocode and two key methods in python in the appendix. All games are available via open source libraries (OpenSpiel, gambit, and GAMUT) or referenced directly in papers (e.g., modified Shapley's game).
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}. We report standard error of the mean.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}. See \S\ref{exp} and Appx.~\ref{app:runtime}.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}.
  \item Did you mention the license of the assets?
    \answerNo{}. The OpenSpiel (\href{https://github.com/deepmind/open_spiel/blob/master/LICENSE}{Apache}), gambit (\href{http://www.gambit-project.org/gambit13/index.html}{GNU license}), and GAMUT (\href{http://gamut.stanford.edu/}{Apache license on download page}) licenses are clearly stated on their websites.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}.
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
